Storage, Accumulation and Deceleration of Secondary Beams for Nuclear Astrophysics

Low-energy investigations on rare ion beams are often limited by the available intensity and purity of the ion species in focus. Here, we present the first application of a technique that combines in-flight production at relativistic energies with subsequent secondary beam storage, accumulation and finally deceleration to the energy of interest. Using the FRS and ESR facilities at GSI, this scheme was pioneered to provide a secondary beam of $^{118}$Te$^{52+}$ for the measurement of nuclear proton-capture at energies of 6 and 7 MeV/u. The technique provided stored beam intensities of about $10^6$ ions at high purity and brilliance, representing a major step towards low-energy nuclear physics studies using rare ion beams.

==> affiliations.tex <==
\address[gsi]{GSI Helmholtzzentrum f\"ur Schwerionenforschung GmbH, Darmstadt, Germany}
\address[edin]{{University of Edinburgh, Edinburgh, United Kingdom}}
\address[guf]{{Goethe Universit\"at, Frankfurt am Main, Germany}}
\address[imp]{{Institute of Modern Physics, Chinese Academy of Sciences, Lanzhou, China}}
\address[triumf]{{TRIUMF, Vancouver, British Columbia, Canada}}
\address[uvic]{{Department of Physics and Astronomy, University of Victoria, Victoria, Canada}}
\address[jlu]{{Justus-Liebig Universit\"at, Gie{\ss}en, Germany}}
\address[lp2i]{{LP2I Bordeaux, CNRS-IN2P3, Gradignan, France}}
\address[aac]{{University of Applied Sciences, Aachen, Germany}}
\address[hij]{{Helmholtz-Institut Jena, Jena, Germany}}
\address[tud]{{Technische Universit\"at Darmstadt, Darmstadt, Germany}}
\address[riken]{{High Energy Nuclear Physics Laboratory, RIKEN, Saitama, Japan}}
\address[usai]{{Department of Physics, Saitama University, Saitama, Japan}}
\address[utsu]{{Tomonaga Center for the History of the Universe, University of Tsukuba, Ibaraki, Japan}}

%\affiliation[atomki]{{Institute for Nuclear Research (MTA Atomki), Debrecen, Hungary}}
%\affiliation[anu]{{Australian National University, Canberra, Australia}}
%\affiliation[spbu]{{St.~Petersburg State University, St. Petersburg, Russia}}
%\affiliation[bau]{{Al-Balqa Applied University, Salt, Jordan}}
%\affiliation[basel]{{Department of Physics, University of Basel, Switzerland}}
%\affiliation[herts]{{Centre for Astrophysics Research, University of Hertfordshire, Hatfield, United Kingdom}}
%\affiliation[mpik]{{Max-Planck-Institut f\"ur Kernphysik (MPIK), Heidelberg, Germany}}
%\affiliation[tub]{{Technische Universit\"at Braunschweig, Braunschweig, Germany}}
%\affiliation[ptb]{{Physikalisch-Technische Bundesanstalt, Braunschweig, Germany}}
%\affiliation[ulb]{{Institut d’Astronomie et d’Astrophysique, Université Libre de Bruxelles, Brussels, Belgium}}


%\newcommand{\gsi}{\affiliation{GSI Helmholtzzentrum f\"ur Schwerionenforschung GmbH, Darmstadt, Germany}}
%\newcommand{\guf}{\affiliation{Goethe Universit\"at, Frankfurt am Main, Germany}}
%\newcommand{\imp}{\affiliation{Institute of Modern Physics, Chinese Academy of Sciences, Lanzhou, China}}
%\newcommand{\edin}{\affiliation{University of Edinburgh, Edinburgh, United Kingdom}}
%\newcommand{\atomki}{\affiliation{Institute for Nuclear Research (MTA Atomki), Debrecen, Hungary}}
%\newcommand{\cenbg}{\affiliation{LP2I Bordeaux, CNRS-IN2P3, Gradignan, France}}
%\newcommand{\jlu}{\affiliation{Justus-Liebig Universit\"at, Gie{\ss}en, Germany}}
%\newcommand{\anu}{\affiliation{Australian National University, Canberra, Australia}}
%\newcommand{\hij}{\affiliation{Helmholtz-Insitut Jena, Jena, Germany}}
%\newcommand{\spbu}{\affiliation{St.~Petersburg State University, St. Petersburg, Russia}}
%\newcommand{\bau}{\affiliation{Al-Balqa Applied University, Salt, Jordan}}
%\newcommand{\basel}{\affiliation{Department of Physics, University of Basel, Switzerland}}
%\newcommand{\herts}{\affiliation{Centre for Astrophysics Research, University of Hertfordshire, Hatfield, United Kingdom}}
%\newcommand{\ptb}{\affiliation{Physikalisch-Technische Bundesanstalt, Braunschweig, Germany}}
%\newcommand{\tud}{\affiliation{Technische Universit\"at Darmstadt, Darmstadt, Germany}}
%\newcommand{\mpi}{\affiliation{Max-Planck-Institut f\"ur Kernphysik (MPIK), Heidelberg, Germany}}
%\newcommand{\tub}{\affiliation{Technische Universit\"at Braunschweig, Braunschweig, Germany}}
%\newcommand{\aac}{\affiliation{University of Applied Sciences, Aachen, Germany}}
%\newcommand{\ulb}{\affiliation{Institut d’Astronomie et d’Astrophysique, Université Libre de Bruxelles, Brussels, Belgium}}
%\newcommand{\triumf}{\affiliation{TRIUMF, Vancouver, British Columbia, Canada}}
%\newcommand{\uvic}{\affiliation{Department of Physics and Astronomy, University of Victoria, Victoria, British Columbia, Canada}}
%\newcommand{\usai}{\affiliation{Department of Physics, Saitama University, Saitama, Japan}}
%\newcommand{\utsu}{\affiliation{Tomonaga Center for the History of the Universe, University of Tsukuba, Ibaraki, Japan}}
